Listen and Move: Improving GANs Coherency in Agnostic Sound-to-Video Generation

Deep generative models have demonstrated the ability to create realistic audiovisual content, sometimes driven by domains of different nature. However, smooth temporal dynamics in video generation is a challenging problem. This work focuses on generic sound-to-video generation and proposes three main features to enhance both image quality and temporal coherency in generative adversarial models: a triple sound routing scheme, a multi-scale residual and dilated recurrent network for extended sound analysis, and a novel recurrent and directional convolutional layer for video prediction. Each of the proposed features improves, in both quality and coherency, the baseline neural architecture typically used in the SoTA, with the video prediction layer providing an extra temporal refinement.

==> figures/silent_frames.tex <==
\begin{subfigure}{0.48\linewidth}
    \centering
    \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mel64-146.png}
    \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mel64-147.png}
    \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mel64-148.png}
    % \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mel64-149.png}
    
    \vspace{0.1cm}
    \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mel64-146.png}
    \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mel64-147.png}
    \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mel64-148.png}
    % \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mel64-149.png}

    \vspace{0.1cm}
    \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mel128-146.png}
    \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mel128-147.png}
    \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mel128-146.png}
    % \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mel128-146.png}
    \caption{From 'silent' 64 mel bins.}
    \end{subfigure}
    \unskip\ \vrule\
    \begin{subfigure}{0.48\linewidth}
    \centering
    \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mfcc-146.png}
    \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mfcc-147.png}
    \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mfcc-148.png}
    % \includegraphics[width=0.318\linewidth, trim={1.0cm 1.8cm 1.0cm 0.2cm}, clip] {assets/silence-frames/seyeon-silence-mfcc-149.png}    
    
    \vspace{0.1cm}
    \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mfcc-146.png}
    \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mfcc-147.png}
    \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mfcc-148.png}
    % \includegraphics[width=0.318\linewidth, trim={1.2cm 0.9cm 1.2cm 1.5cm}, clip] {assets/silence-frames/jacob-silence-mfcc-149.png}
    
    \vspace{0.1cm}
    \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mfcc-146.png}
    \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mfcc-147.png}
    \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mfcc-148.png}
    % \includegraphics[width=0.318\linewidth, trim={0.5cm 0.6cm 0.5cm 0.4cm}, clip] {assets/silence-frames/obama-silence-mfcc-149.png}
    \caption{From 'silent' 20 MFCCs.}
    \end{subfigure}

==> tables/mel_vs_mfcc.tex <==
    \resizebox{1.0\linewidth}{!}
    {
    \begin{tabular}{lccccccccccc}
    % \toprule
    \cmidrule{2-12}
    &\multicolumn{3}{c}{\textit{Seyeon}}    &
    &\multicolumn{3}{c}{\textit{Jacob}}     &
    &\multicolumn{3}{c}{\textit{Barak}}     \\
    \cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
    &FID ($\downarrow$) & PSNR  & SSIM &
    &FID ($\downarrow$) & PSNR  & SSIM &
    &FID ($\downarrow$) & PSNR  & SSIM     \\
    % \midrule
    % MFCC 20 & $47.3\pm44.2$ &$20.9\pm1.8$ &$0.85\pm0.05$ &&$95.1\pm46.3$ &$22.7\pm1.5$ &$0.89\pm0.04$ &&$29.1\pm04.0$ &$20.6\pm2.4$ &$0.67\pm0.08$ \\ 
    % Mel 64  & $52.3\pm18.7$ &$21.1\pm1.7$ &$0.85\pm0.04$ &&$89.4\pm13.7$ &$22.4\pm1.0$ &$0.88\pm0.02$ &&$54.4\pm15.8$ &$20.1\pm2.2$ &$0.66\pm0.07$ \\
    % % Mel 128 & $88.7\pm27.7$ &$20.8\pm1.6$ &$0.84\pm0.05$ &&$75.1\pm15.7$ &$22.6\pm1.0$ &$0.88\pm0.02$ &&$43.5\pm18.1$ &$20.2\pm2.3$ &$0.66\pm0.08$ \\
    % \midrule
    % Mel 64 Encoded &$36.7\pm10.8$ & $20.7\pm1.8$ & $0.86\pm0.05$ && $75.5\pm18.8$ & $19.9\pm1.8$ & $0.82\pm0.05$ && $69.7\pm8.2$ & $18.2\pm2.2$ & $0.52\pm0.07$  \\
    % \bottomrule
    \midrule
    MFCC & $47\pm44$ &$20.9\pm1.8$ &$0.85\pm0.05$ &&$95\pm46$ &$22.7\pm1.5$ &$0.89\pm0.04$ &&$29\pm04$ &$20.6\pm2.4$ &$0.67\pm0.08$ \\ 
    Mel & $52\pm19$ &$21.1\pm1.7$ &$0.85\pm0.04$ &&$89\pm14$ &$22.4\pm1.0$ &$0.88\pm0.02$ &&$54\pm16$ &$20.1\pm2.2$ &$0.66\pm0.07$ \\
    \midrule
    Mel+AE &$36\pm19$ & $21.0\pm1.8$ & $0.86\pm0.05$ && $75\pm40$ & $19.9\pm1.8$ & $0.82\pm0.05$ && $75\pm10$ & $18.3\pm2.1$ & $0.53\pm0.07$  \\
    \bottomrule    
    \end{tabular}
    }

==> tables/mel_vs_mfcc_FSD50K.tex <==
    \resizebox{0.75\linewidth}{!}
    {
    \begin{tabular}{lccc}
    \toprule
    % \cmidrule{2-6}
    FID ($\downarrow$)
    &\textit{Seyeon}
    &\textit{Jacob}
    &\textit{Barak}\\
    % \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
    \midrule
    MFCC         &$216\pm90$    &$324\pm83$   &$116\pm96$\\
    Mel           &$114\pm59$    &$143\pm71$  &$112\pm88$\\
    % Mel 128       &$163\pm51$    &$154\pm83$  &$97\pm86$ \\
    \midrule
    Mel+AE &$71\pm53$      &$71\pm53$  &$71\pm53$ \\
    \bottomrule
    \end{tabular}
    }

==> tables/routes_and_seqlength.tex <==
    \resizebox{1.0\linewidth}{!}
    {
    \begin{tabular}{ccccc}
    % \toprule
    \cmidrule{3-5}
     & & FID ($\downarrow$) & PSNR  & SSIM \\
    \midrule
    \multirow{3}{*}{\rotatebox[origin=c]{90}{$L=8$}} \
    & MfS & $93.2\pm67.2$ & $19.9\pm2.0$ & $0.81\pm0.07$ \\
    & SaC & $52.7\pm30.0$ & $20.2\pm1.6$ & $0.82\pm0.07$ \\
    & MfS+SaC & $\mathbf{23.5}\pm11.4$ & $\mathbf{20.5}\pm1.5$ & $\mathbf{0.85}\pm0.04$ \\
    \midrule
    \multirow{3}{*}{\rotatebox[origin=c]{90}{$L=16$}} \
    & MfS & $136.3\pm56.4$ & $20.1\pm1.9$ & $0.77\pm0.08$ \\
    & SaC & $69.6\pm19.2$ & $20.9\pm1.7$ & $0.84\pm0.05$ \\
    & MfS+SaC & $\mathbf{36.6}\pm8.5$ & $\mathbf{21.5}\pm1.7$ & $\mathbf{0.86}\pm0.04$ \\
    \midrule
    \multirow{3}{*}{\rotatebox[origin=c]{90}{$L=32$}} \
    & MfS & $58.2\pm16.1$ & $21.6\pm1.6$ & $0.85\pm0.04$ \\
    % & SaC & $\mathbf{38.3}\pm10.1$ & $21.3\pm1.7$ & $\mathbf{0.86}\pm0.04$ \\
    & SaC & $46.4\pm19.0$ & $\mathbf{21.7}\pm1.7$ &  $0.86\pm0.04$ \\
    % & MfS+SaC & $57.5\pm21.2$ & $21.5\pm1.7$ & $\mathbf{0.86}\pm0.03$ \\
    % & MfS+SaC & $56.0\pm17.4$ & $\mathbf{21.8}\pm1.8$ & $\mathbf{0.87}\pm0.03$ \\
    & MfS+SaC & $\mathbf{40.7}\pm30.09$ & $\mathbf{21.7}\pm1.7$ & $\mathbf{0.87}\pm0.04$ \\
    \midrule
    \multirow{3}{*}{\rotatebox[origin=c]{90}{$L=64$}} \
    & MfS & $\mathbf{21.3}\pm4.3$ & $\mathbf{22.9}\pm1.8$ & $\mathbf{0.90}\pm0.02$ \\
    & SaC & $23.3\pm7.1$ & $21.9\pm1.1$ & $0.88\pm0.03$ \\
    % & MfS+SaC & $21.5\pm7.6$ & $22.6\pm1.9$ & $\mathbf{0.90}\pm0.02$ \\
    & MfS+SaC & $23.8\pm6.5$ & $22.6\pm1.9$ & $\mathbf{0.90}\pm0.02$ \\
    % \midrule
    \bottomrule
    \end{tabular}
    }

==> tables/suburmp.tex <==
% Quality metrics for checkpoint: ../20230214122705-suburmp-cello-256-route_rnngen-motion_L3basic-vp_dir-cond_gen/checkpoints/0200000_Gn.model
% FVD:  1746.5 ± 949.2
% FID:  29.8 ± 4.3
% MSE:  0.02950 ± 0.00854
% PSNR: 15.5 ± 1.2
% SSIM: 0.61 ± 0.04
% LPIPS:0.20 ± 0.04

% Quality metrics for checkpoint: ../20230214122608-suburmp-trombone-256-route_rnngen-motion_L3basic-vp_dir-cond_gen/checkpoints/0200000_Gn.model
% FVD:  4528.2 ± 760.1
% FID:  252.9 ± 15.6
% MSE:  0.08079 ± 0.00302
% PSNR: 10.9 ± 0.2
% SSIM: 0.31 ± 0.01
% LPIPS:0.55 ± 0.01

                        CELLO                       TROMBONE
                    PSNR         SSIM           PSNR         SSIM
EBDN [3]        &   13.553      0.246           12.358      0.225
vid2vid [36]    &   13.284      0.331           9.600       0.204 
Let's Play Music&   17.073       0.563          15.910      0.397
Ours            &   15.5 ± 1.2  0.61 ± 0.04     10.9 ± 0.2  0.31 ± 0.01

